TeacherLM: Teaching to Fish Rather Than Giving the Fish, Language Modeling Likewise

Large Language Models (LLMs) exhibit impressive reasoning and data augmentation capabilities in various NLP tasks. However, what about small models? In this work, we propose TeacherLM-7.1B, capable of annotating relevant fundamentals, chain of thought, and common mistakes for most NLP samples, which makes annotation more than just an answer, thus allowing other models to learn "why" instead of just "what". The TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing most models with over 100B parameters. Even more remarkable is its data augmentation ability. Based on TeacherLM-7.1B, we augmented 58 NLP datasets and taught various student models with different parameters from OPT and BLOOM series in a multi-task setting. The experimental results indicate that the data augmentation provided by TeacherLM has brought significant benefits. We will release the TeacherLM series of models and augmented datasets as open-source.

==> content/0-Abstract-2023012603.tex <==
Large Language Models (LLMs) exhibit impressive reasoning and data augmentation capabilities in various NLP tasks. However, what about small models? In this work, we propose TeacherLM-7.1B, capable of generating relevant fundamentals, chain of thought, and common mistakes for most NLP samples. This makes the annotation more than just an answer, thus allowing the model to learn ``why'' instead of just ``what''. The TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing most models with over 100B parameters. Even more remarkable is its data augmentation ability. Based on TeacherLM-7.1B, we augmented 58 NLP datasets and taught various student models with different parameters from OPT and BLOOM series in a multi-task setting. The experimental results indicate that the data augmentation provided by TeacherLM has brought significant benefits. We will release the TeacherLM series of models and augmented datasets as open-source.

% Large Language Models (LLMs) exhibit impressive reasoning and data augmentation capabilities in various NLP tasks. However, what about small models? In this work, we propose TeacherLM-7.1B, capable of generating relevant fundamentals, chain of thought, and common mistakes for most NLP samples. This process makes annotation more than just an answer, thus allowing other models to learn ``why'' instead of just ``what''. The TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing most models with over 100B parameters. Even more remarkable is its data augmentation ability. Based on TeacherLM-7.1B, we augmented 58 NLP datasets and taught various student models with different parameters from OPT and BLOOM series in a multi-task setting. The experimental results indicate that TeacherLM's data augmentation gains clear benefits. We will release the TeacherLM series of models and augmented datasets as open-source.

==> content/0-Abstract.tex <==
Large Language Models (LLMs) exhibit impressive reasoning and data augmentation capabilities in various NLP tasks. However, what about small models? In this work, we propose TeacherLM-7.1B, which can explain most NLP samples through fundamentals, chain of thought, and common mistakes, making the annotation more than just an answer. The TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing most of the hundred-billion-parameter models. More important and remarkable is its data augmentation ability. We enhanced 58 NLP datasets by TeacherLM-7.1B and conducted multi-task training, with experiments demonstrating significant gains of over 10\% [xxx] on multiple benchmarks for various parameter models of OPT and BLOOM. Furthermore, compared to the manually annotated rationales and the latest GPT model text-davinci-003's explanations, ours have clear advantages on multiple tasks.    % 加入引用
%Furthermore, our explanation has clear advantages on multiple tasks compared to the manually annotated rationale and the latest GPT model text-Davinci-003's analysis.
% 是否要统一 manually annotated rationale 以及 explanation？我认为不应该用 explanation，就是全程用 analysis
We will release the TeacherLM series of models and augmented datasets as open-source [xxx].
% TODO Enhenced 和 augmentation 是混用，还是只用一个？
% on multiple tasks 是什么意思，这里的 multiple 是指多个么？可以改成 single datasets 么？
% 开篇完全不提为什么要做增强么？

==> content/01-Introduction-zmj-2023012601.tex <==
Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. Compared to the increase in model size, an essential thing for achieving a deeper understanding of language is to utilize data effectively. Unfortunately, most NLP datasets have simple input-output pairs inconsistent with the data seen during the pre-training of language models. As a result, directly fine-tuning such data is not sufficient for the model to fully understand the content of the samples, inducing difficulty in fully utilizing its learning capabilities. Thus, two leading data augmentation strategies have emerged to address this issue, including task-level and instance-level approaches.

% Unfortunately, most NLP datasets have simple input-output pairs, inconsistent with the pre-training data of language models. As a result, directly fine-tuning such data is not sufficient for the model to fully understand the content of the samples, inducing difficulty in fully utilizing its learning capabilities. Thus, two leading data augmentation strategies have emerged to address this issue, including task-level and instance-level approaches.

% x小修小改了一些语句

In task-level data augmentation, the aim is to map any natural language task into multiple human-readable prompted forms with diverse wording \cite{wei2021finetuned,bach2022promptsource,wang2022super}. Furthermore, combining task-level augmentation with multi-task training leads to a more comprehensive ability. Fine-tuning a pre-trained model on this multi-task mixture covering various tasks \cite{sanh2021multitask,chung2022scaling,muennighoff2022crosslingual,iyer2022opt} induces the language model a more substantial zero-shot and few-shot capabilities.

Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting the enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance each sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models \cite{borgeaud2021improving,izacard2022few} utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs \cite{wang2021towards,ho2022large} can use their solid zero-shot ability to enhance data for each sample based on different prompts. Nevertheless, these two methods bring huge usage costs, and some of the best current work is not open source.

In order to reduce the cost of data augmentation, in this work, we propose to open-source a series of small TeacherLM models that rival human annotation and large models. The adage goes, "It is better to teach someone how to fish than to give them the fish." This applies to language models as well. Two perspectives primarily drive our approach. Firstly, we believe that the real need for enhancement in a dataset lies in each sample's label, where the model should learn "why" instead of just remembering "what". Our goal is to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization and towards a more holistic understanding to break through current limitations imposed on language model capabilities. Secondly, language models should mimic humans' learning process by simultaneously learning each sample's relevant fundamentals, chain of thought, and common mistakes to understand the training objectives more comprehensively.

% The adage goes, "It is better to teach someone how to fish than to give them the fish, " which also applies to language models. 小修小补
% drive -> navigate
% Firstly, we believe that the real need for enhancement in a dataset lies in each sample's label, where the model should learn "why" instead of just remembering "what." Our goal is to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization towards a more holistic understanding to break through current limitations imposed on language model capabilities. Secondly, language models should mimic humans' learning process by simultaneously learning each sample's relevant fundamentals, chain of thought, and common mistakes to understand the training objectives more comprehensively.

To achieve this, we define the learning process as comprising three dimensions: fundamental, chain of thought, and common mistake. Our ultimate goal is to annotate this information for every sample in an NLP dataset. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. Furthermore, we combined manual annotation and STaR [xxx] strategy to construct a complete ``\textit{\{Question\}\text{ }\{Answer\}\text{ }\{Fundamentals\}\text{ }\{Chain of Thought\}\text{ }\{Common Mistakes\}}" five-element training object for each sample.

% 这里改用了斜体

In sum, our key contributions are:

\begin{itemize}
\item \textbf{Comprehensive}:
TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information tailored to the task's characteristics and allowing each task to learn the most relevant knowledge.

\item \textbf{Generalizability}:
TeacherLM is suitable for a variety of datasets and models. As shown in the figure, we augmented 58 NLP datasets and taught various student models with different parameters from opt and bloom series in a multi-task setting. Compared to non-augmented versions, the experimental results indicate that the data augmentation provided by TeacherLM has brought significant benefits.

\item \textbf{Fight big with small}:
TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing most models with over 100B parameters.

\item \textbf{Cost friendly}:
TeacherLM-7.1B has only 7.1 billion parameters; compared to models such as text-davinci-003 [xxx], it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.

\item \textbf{Open source}:
We will release the TeacherLM series of models and augmented datasets as open-source.
\end{itemize}

==> content/01-Introduction-zmj-pre.tex <==
Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. Compared to the increase in model size, an essential thing for achieving a deeper understanding of language is to utilize data effectively. The key to enhancing the capabilities of language models lies in effectively teaching them to comprehend and use the data provided, with related work primarily divided into task-level and instance-level. In task-level data augmentation, the aim is to map any natural language task into multiple human-readable prompted forms with diverse wording \cite{wei2021finetuned,bach2022promptsource,wang2022super}. The combination with multi-task training leads to a more comprehensive ability, fine-tuning a pre-trained model on this multitask mixture covering a wide variety of tasks \cite{sanh2021multitask,chung2022scaling,muennighoff2022crosslingual,iyer2022opt}, pushes the generality of language models to a new heights, and has strong zero-shot and few-shot capabilities.
%这一段最后一整句有点难读 还有a new heights, multitask和multi-task
% map 是映射的意思么？
% The combination 改为 Furthermore, combining task-level enhencedment with...
% 统一 pretrain 和 multi-task
% Furthermore, combining task-level enhancement with multi-task training leads to a more comprehensive ability. Finetuning a pre-trained model on this multi-task mixture covering a wide variety of tasks pushes the generality of language models to new heights and has strong zero-shot and few-shot capabilities.
% 感觉用entity这个词不是很好
% 删掉corresponding;  Large language model改复数 ; 删掉its own 中的own
% 

Each sample represents an individual entity, and the enhancement brought about by treating the entire dataset as a whole using a unified method of data augmentation is limited. The most effective approach is to enhance each sample individually based on its unique characteristics. A new stage will flourish in instance-level data enhancement. Retrieval-based pre-trained language models utilize small models in conjunction with a massive database to introduce more corresponding relevant knowledge for each sample \cite{borgeaud2021improving,izacard2022few}. Large language model can use its own strong zero-shot ability to enhance data for each sample based on different prompts \cite{wang2021towards,ho2022large}. However, these two methods bring huge usage costs, and some of the best current work is not open source.
% Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting the enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance each sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models [xxx] utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs [xxx] can use their solid zero-shot ability to enhance data for each sample based on different prompts. Nevertheless, these two methods bring huge usage costs, and some of the best current work is not open source.
% 主要的修改逻辑：1. 在 Each sample 这一句加入了转折；2. 第二句同样加入转折，且把第三句用 flouring 串接起来；4. 再在 Retrieval-based pre-trained language models 前加入转折，LLMs 前同理。

In order to reduce the cost of data augmentation, this work presents an open-source series of TeacherLM small models that rival human annotation and large language models. ``It is better to teach someone how to fish than to give them the fish." This adage applies to language models as well. The question then arises, how can we effectively teach a language model? The answer is to allow the language model to learn in a way that mimics human learning. Simply providing a label with a straightforward answer is insufficient for many NLP tasks. Instead, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization and towards a more holistic understanding to break through the limitations currently imposed on language model capabilities.

In order to achieve this, we define the learning process as comprising three dimensions: fundamental, chain of thought, and common mistake. Our ultimate goal is to annotate this information for every sample in an NLP dataset. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. And combined manual annotation and STaR strategy to construct a complete question-answer-fundamental-chain of thought-common mistake five-element for each sample.

% ----------------

% Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. However, ``It is better to teach someone how to fish than to give them the fish." Compared to the increase in model size, an essential thing for enhancing the capabilities of language models lies in allowing the language model to learn in a way that mimics human learning. Specifically, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization towards a more holistic understanding to break through the limitations currently imposed on language model capabilities. However, many NLP tasks with a simple label of answer are insufficient for this purpose, requiring data augmentation, inducing primary related work divided into task-level or instance-level data augmentation.

% In task-level data augmentation [xxx], the aim is to map natural language tasks into multiple human-readable prompted forms with diverse wording. Also, combining task-level enhancement with multi-task training leads to a more comprehensive ability. Finetuning a pre-trained model on this multi-task mixture covering a wide variety of tasks pushes the generality of language models to new heights and has strong zero-shot and few-shot capabilities.

% Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting task-level enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance every sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models [xxx] utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs [xxx] can also use their solid zero-shot ability to enhance each sample based on different prompts.

% Nevertheless, these two methods bring huge usage costs, and some of the best current works are not open source. Thus, this work presents an open-source series of TeacherLM small models that rival human annotation and large language models to reduce the limitation of current instance-level data augmentation methods. 

% In order to achieve this, we define the learning process as comprising three dimensions: fundamentals, the chain of thought(CoT), and common mistakes. Our ultimate goal is to annotate this information for every sample in NLP datasets. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. Furthermore, we combined manual annotations and STaR [xxx] strategy to construct a $\rm Question-Answer-Fundamentals-Chain of Thought-Common Mistakes$ five-element training data for each sample.
% In sum, our key contributions are:

% --------------------

\begin{itemize}
\item \textbf{Comprehensive}:
TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information that can be tailored to the characteristics of the task, allowing each task to learn the most suitable knowledge.
% 这里用explain是啥意思
\item \textbf{Generalizability}:
TeacherLM is suitable for a variety of datasets and models. We enhanced 59 NLP datasets and then used various parameter models of Opt and Bloom as student models for multi-task training on the enhanced data, as shown in the figure. Compared to non-enhanced versions, the zero-shot scores for MMLU, QASC, SenseMaking, CREAK, StrategyQA, and ECQA improved by more than 10\%.
\item \textbf{Fight big with small}:
TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing the majority of the hundreds of billions of parameter models.

\item \textbf{Beyond human annotation}:
On the QASC, SenseMaking, CREAK, StrategyQA, and ECQA datasets, TeacherLM-7.1B has demonstrated the ability to enhance data beyond human annotation and has some competitiveness compared to text-davinci-003, and to a great extent mitigates the CoT hurt situation.
% 这里说超越人工，应该不是这几个都超过了
\item \textbf{Low cost and low resource consumption}:
TeacherLM-7.1B has only 7.1 billion parameters; compared to models such as text-davinci-003, it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.

\item \textbf{Open source}:
We will release the TeacherLM series of models and augmented datasets as open-source.
\end{itemize}

==> content/01-Introduction-zmj.tex <==
Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. 
%
Compared to the increase in model size, an essential thing for achieving a deeper understanding of language is to utilize data effectively. 
% We have to mention the importance of adaptation for pre-trained LMs.
The key to exploiting the usability of language models for downstream tasks lies in effectively adapting them to understand the context of the target problem. Current adaptation approaches fall into two categories: task-level and instance-level adaptation. 
% Task-level adaptation
In task-level adaptation, a language-based template for each task is proposed so that the pre-trained language model can apply to the downstream tasks via further tuning. For example, GPT-3 xxxxx and FLAN xxxx zero-shot settings.
%

% Instance-level adaptation
For instance-level adaptation, instead of using the same template for all data, the template is specific for each of the data.
%
Retrieval-based pre-trained language models utilize small models in conjunction with a massive database to introduce more corresponding relevant knowledge for each sample. Large language models can use their own strong zero-shot ability to enhance data for each sample based on different prompts. However, these two methods bring huge usage costs, and some of the best current work is not open source. 

% Comapre both settings, and state why instance-level is better.
While, instance-level xxx advantage over task level xxx. It is costly to create a large set of high quality instance-level adaptation templates. In order to reduce the annotation cost.
% Introduce our work
We present an a series of TeacherLM models that rival human annotation and large language models. We aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization and towards a more holistic understanding to break through the limitations currently imposed on language model capabilities.

In order to achieve this, we define the learning process as comprising three dimensions: fundamental, chain of thought, and common mistake. Our ultimate goal is to annotate this information for every sample in an NLP dataset. To ensure that TeacherLM has strong zero-shot capabilities for most 5 natural language processing tasks, we have collected 2 million samples from multiple domains for training. And combined manual annotation and STaR strategy to construct a complete question-answer-fundamental-chain of thought-common mistake five-element for each sample.

%What we achieved? What kind of problems we solved.

In sum, our key contributions are:

\begin{itemize}
\item \textbf{Comprehensive}:
TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information that can be tailored to the characteristics of the task, allowing each task to learn the most suitable knowledge.

\item \textbf{Generalizability}:
TeacherLM is suitable for a variety of datasets and models. We enhanced 59 NLP datasets and then used various parameter models of Opt and Bloom as student models for multi-task training on the enhanced data, as shown in the figure. Compared to non-enhanced versions, the zero-shot scores for MMLU, QASC, SenseMaking, CREAK, StrategyQA, and ECQA improved by more than 10\%.
\item \textbf{Fight big with small}:
TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing the majority of the hundreds of billions of parameter models.

\item \textbf{Beyond human annotation}:
On the QASC, SenseMaking, CREAK, StrategyQA, and ECQA datasets, TeacherLM-7.1B has demonstrated the ability to enhance data beyond human annotation and has some competitiveness compared to text-davinci-003, and to a great extent mitigates the CoT hurt situation.

\item \textbf{Low cost and low resource consumption}:
TeacherLM-7.1B has only 7.1 billion parameters; compared to models such as text-davinci-003, it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.

\item \textbf{Open source}:
We will release the TeacherLM series of models and augmented datasets as open-source.
\end{itemize}

==> content/01-Introduction.tex <==
% Starting with the introduction of background  
Large Language models have shown unprecedented results in many NLP tasks. The more exciting thing is that large language models take in-context learning to a new level. 

% Next, we should talk about the importance of COT in some reasoning tasks.
However, current large language models struggle in reasoning-intensive tasks such as arithmetic, commonsense, and symbolic reasoning. There have been attempts that utilize CoT (Chain-of-Thought) in order to mimic humans for solving complex reasoning tasks. A chain of thought is a series of intermediate natural language reasoning steps for yielding the final prediction. FLAN uses CoT data for instructional fine-tuning. Wei etal \cite{} proposed to utilize chain-of-thought as prompts to improve the ability of large language models to perform complex reasoning. 

% What are the limitations of the current usage of CoT?  Limited by the number of data? As well as the content of the existing CoT data?
The problems of FLAN are xxxx. The problems of \cite{} are xxxx.

% Introduce what we proposed.
We propose TeacherLM  for dataset augmentation that can generate CoT annotations for a wide range of conventional NLP datasets? 
% How we achieved this, give some details here.
We create a large-scale CoT dataset and propose a training paradigm. 

% What are the effects of TeacherLM? How we improve student models with it? 

% Summarize contributions.




==> content/Intro_by_zcy.tex <==
% % ----------------

Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. However, ``It is better to teach someone how to fish than to give them the fish." Compared to the increase in model size, an essential thing for enhancing the capabilities of language models lies in allowing the language model to learn in a way that mimics human learning. Specifically, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization towards a more holistic understanding to break through the limitations currently imposed on language model capabilities. However, many NLP tasks with a simple label of answer are insufficient for this purpose, requiring data augmentation, inducing primary related work divided into task-level or instance-level data augmentation.

In task-level data augmentation [xxx], the aim is to map natural language tasks into multiple human-readable prompted forms with diverse wording. Also, combining task-level enhancement with multi-task training leads to a more comprehensive ability. Finetuning a pre-trained model on this multi-task mixture covering a wide variety of tasks pushes the generality of language models to new heights and has strong zero-shot and few-shot capabilities.

Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting task-level enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance every sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models [xxx] utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs [xxx] can also use their solid zero-shot ability to enhance each sample based on different prompts.

Nevertheless, these two methods bring huge usage costs, and some of the best current works are not open source. Thus, this work presents an open-source series of TeacherLM small models that rival human annotation and large language models to reduce the limitation of current instance-level data augmentation methods. 

In order to achieve this, we define the learning process as comprising three dimensions: fundamentals, the chain of thought(CoT), and common mistakes. Our ultimate goal is to annotate this information for every sample in NLP datasets. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. Furthermore, we combined manual annotations and STaR [xxx] strategy to construct a ``\textit{\{Question\}\text{ }\{Answer\}\text{ }\{Fundamentals\}\text{ }\{Chain of Thought\}\text{ }\{Common Mistakes\}}'' five-element training data for each sample.

% $ \rm \{Question-Answer-Fundamentals-\text{Chain of Thought}-\text{Common Mistakes}\}$

In sum, our key contributions are:

% --------------------

\begin{itemize}
\item \textbf{Comprehensive}:
TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information tailored to the task's characteristics and allowing each task to learn the most relevant knowledge.
% 这里用explain是啥意思
\item \textbf{Generalizability}:
TeacherLM is suitable for a wide variety of datasets and models. As shown in figure [xxx], we enhanced 58 NLP datasets and then used various models of Opt [xxx] and Bloom [xxx] as student models for multi-task training on the enhanced data. Compared to non-enhanced versions, the zero-shot scores of student models on MMLU, QASC, SenseMaking, CREAK, StrategyQA, and ECQA improved by more than 10\%.

\item \textbf{Fight big with small}:
The teacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing the majority of the hundreds of billions of parameter models.

\item \textbf{Beyond human annotation}:
On the CREAK, StrategyQA, and ECQA datasets, TeacherLM-7.1B has demonstrated the ability to enhance data beyond human annotation and has some competitiveness compared to the current most powerful GPT-3 model text-davinci-003 and, to a great extent, mitigates the CoT hurt situation.
% 这里真的是这个故事么？此外，我觉得这里小标题没概括好
\item \textbf{Friendly to use}:
TeacherLM-7.1B has only 7.1 billion parameters; compared to LLMs, it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.

\item \textbf{Open source}:
We will release the TeacherLM series of models and augmented datasets as open-source.
\end{itemize}

% -------------------------

% Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. Compared to the increase in model size, an essential thing for achieving a deeper understanding of language is to utilize data effectively. A key to enhancing the capabilities of language models lies in virtually teaching them to understand comprehensive training data. However, simply providing a label with a straightforward answer is insufficient for many NLP tasks requiring data augmentation, inducing primarily related work divided into task-level or instance-level data augmentation. In task-level data augmentation, the aim is to map any natural language task into multiple human-readable prompted forms with diverse wording \cite{wei2021finetuned,bach2022promptsource,wang2022super}. The combination with multi-task training leads to a more comprehensive ability, fine-tuning a pre-trained model on this multitask mixture covering a wide variety of tasks \cite{sanh2021multitask,chung2022scaling,muennighoff2022crosslingual,iyer2022opt}, pushes the generality of language models to a new heights, and has strong zero-shot and few-shot capabilities.

%这一段最后一整句有点难读 还有a new heights, multitask和multi-task
% map 是映射的意思么？
% The combination 改为 Furthermore, combining task-level enhencedment with...
% 统一 pretrain 和 multi-task
% Furthermore, combining task-level enhancement with multi-task training leads to a more comprehensive ability. Finetuning a pre-trained model on this multi-task mixture covering a wide variety of tasks pushes the generality of language models to new heights and has strong zero-shot and few-shot capabilities.
% 感觉用entity这个词不是很好
% 删掉corresponding;  Large language model改复数 ; 删掉its own 中的own
% 

% Each sample represents an individual entity, and the enhancement brought about by treating the entire dataset as a whole using a unified method of data augmentation is limited. The most effective approach is to enhance each sample individually based on its unique characteristics. A new stage will flourish in instance-level data enhancement. Retrieval-based pre-trained language models utilize small models in conjunction with a massive database to introduce more corresponding relevant knowledge for each sample \cite{borgeaud2021improving,izacard2022few}. Large language model can use its own strong zero-shot ability to enhance data for each sample based on different prompts \cite{wang2021towards,ho2022large}. However, these two methods bring huge usage costs, and some of the best current work is not open source.
% Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting the enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance each sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models [xxx] utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs [xxx] can use their solid zero-shot ability to enhance data for each sample based on different prompts. Nevertheless, these two methods bring huge usage costs, and some of the best current work is not open source.
% 主要的修改逻辑：1. 在 Each sample 这一句加入了转折；2. 第二句同样加入转折，且把第三句用 flouring 串接起来；4. 再在 Retrieval-based pre-trained language models 前加入转折，LLMs 前同理。

% In order to reduce the cost of data augmentation, this work presents an open-source series of TeacherLM small models that rival human annotation and large language models. ``It is better to teach someone how to fish than to give them the fish." This adage applies to language models as well. The question then arises, how can we effectively teach a language model? The answer is to allow the language model to learn in a way that mimics human learning. Simply providing a label with a straightforward answer is insufficient for many NLP tasks. Instead, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization and towards a more holistic understanding to break through the limitations currently imposed on language model capabilities.

% In order to achieve this, we define the learning process as comprising three dimensions: fundamental, chain of thought, and common mistake. Our ultimate goal is to annotate this information for every sample in an NLP dataset. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. And combined manual annotation and STaR strategy to construct a complete question-answer-fundamental-chain of thought-common mistake five-element for each sample.

% ----------------

% Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. However, ``It is better to teach someone how to fish than to give them the fish." Compared to the increase in model size, an essential thing for enhancing the capabilities of language models lies in allowing the language model to learn in a way that mimics human learning. Specifically, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization towards a more holistic understanding to break through the limitations currently imposed on language model capabilities. However, many NLP tasks with a simple label of answer are insufficient for this purpose, requiring data augmentation, inducing primary related work divided into task-level or instance-level data augmentation.

% In task-level data augmentation [xxx], the aim is to map natural language tasks into multiple human-readable prompted forms with diverse wording. Also, combining task-level enhancement with multi-task training leads to a more comprehensive ability. Finetuning a pre-trained model on this multi-task mixture covering a wide variety of tasks pushes the generality of language models to new heights and has strong zero-shot and few-shot capabilities.

% Though task-level enhancement has pushed the language model's generalizability to a new height, each sample represents an individual entity, limiting task-level enhancement by treating the entire dataset using a unified data augmentation method. Hence a more effective approach is to enhance every sample individually based on its unique characteristics, with a new stage flourishing in instance-level data enhancement. For this approach, retrieval-based pre-trained language models [xxx] utilize small models in conjunction with a massive database to introduce more relevant knowledge for each sample. Meanwhile, LLMs [xxx] can also use their solid zero-shot ability to enhance each sample based on different prompts.

% Nevertheless, these two methods bring huge usage costs, and some of the best current works are not open source. Thus, this work presents an open-source series of TeacherLM small models that rival human annotation and large language models to reduce the limitation of current instance-level data augmentation methods. 

% In order to achieve this, we define the learning process as comprising three dimensions: fundamentals, the chain of thought(CoT), and common mistakes. Our ultimate goal is to annotate this information for every sample in NLP datasets. To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. Furthermore, we combined manual annotations and STaR [xxx] strategy to construct a $\rm Question-Answer-Fundamentals-Chain of Thought-Common Mistakes$ five-element training data for each sample.
% In sum, our key contributions are:

% --------------------

% \begin{itemize}
% \item \textbf{Comprehensive}:
% TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information that can be tailored to the characteristics of the task, allowing each task to learn the most suitable knowledge.
% % 这里用explain是啥意思
% \item \textbf{Generalizability}:
% TeacherLM is suitable for a variety of datasets and models. We enhanced 59 NLP datasets and then used various parameter models of Opt and Bloom as student models for multi-task training on the enhanced data, as shown in the figure. Compared to non-enhanced versions, the zero-shot scores for MMLU, QASC, SenseMaking, CREAK, StrategyQA, and ECQA improved by more than 10\%.
% \item \textbf{Fight big with small}:
% TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing the majority of the hundreds of billions of parameter models.

% \item \textbf{Beyond human annotation}:
% On the QASC, SenseMaking, CREAK, StrategyQA, and ECQA datasets, TeacherLM-7.1B has demonstrated the ability to enhance data beyond human annotation and has some competitiveness compared to text-davinci-003, and to a great extent mitigates the CoT hurt situation.
% % 这里说超越人工，应该不是这几个都超过了
% \item \textbf{Low cost and low resource consumption}:
% TeacherLM-7.1B has only 7.1 billion parameters; compared to models such as text-davinci-003, it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.

% \item \textbf{Open source}:
% We will release the TeacherLM series of models and augmented datasets as open-source.
% \end{itemize}


==> content/compare_with_human.tex <==
In section ~\ref{sec:student model}, we enhanced 59 NLP datasets and conducted multi-task training, with remarkable gains for various models. To further reveal the TeacherLM's data augmentation ability, we continue to enhance single NLP datasets and compare TeacherLM's performance with human annotations and the latest GPT3 model text-davinci-003.

% 加入引用

\subsection{Finetuning Settings}
\subsubsection{Finetuning Data}
\paragraph{Dataset composition.} To accurately evaluate the TeacherLM’s augmentation ability on single tasks, we chose five datasets with manually annotated CoT, including CREAK, QASC, ECQA, SenseMaking, and StrategyQA. We reassembled the data in the original dataset and generated its question, answer, and human rationale, as shown in Figure ~\ref{fig:dataset}. To avoid the different split settings among datasets, we divided all datasets into the training set (85\%) and test set (15\%).
% TODO: 加入引用

\input{figure/five_dataset.tex}
% TODO: 图片格式挂了

\paragraph{Augmentation and fields denotation.} Each dataset contains the full question, answer, and manually annotated CoT for all examples. we denote ``Q: \{question\} A: The answer is \{answer\}" as \textbf{Text} and the manually annotated CoT as \textbf{manual}. Then, we input ``\{Text\} Let's think step by step.", ``\{Text\} The common mistakes are:" and ``\{Text\} The fundamental of this question is:" to the TeacherLM in turn, denoting its three outputs as \textbf{CoT}, \textbf{error}, and \textbf{fundamental}. For comparison with the GPT3, we input the same prompts to the text-davinci-003 and denote its three outputs as \textbf{davinci-CoT}, \textbf{davinci-error}, and \textbf{davinci-fundamental}. 

% TODO：这里需要詹老师说的那个美观标记
\subsubsection{Finetue Prompts}
Following the denotation above, we construct eight finetune task types for each dataset. 

\begin{itemize}
\item \textbf{text}: ``\{Text\}"
\item \textbf{manual-tail}: ``\{Text\} Let’s think step by step. \{manual\}"
\item \textbf{cot-tail}: ``\{Text\} Let’s think step by step. \{CoT\}"
\item \textbf{fundamental-tail}: ``\{Text\} The fundamental of this question is: \{fundamental\}"
\item \textbf{error-tail}: ``\{Text\} The common mistakes are: \{error\}"
\item \textbf{davinci-cot-tail}: ``\{Text\} Let’s think step by step. \{davinci-CoT\}"
\item \textbf{davinci-fundamental-tail}: ``\{Text\} The fundamental of this question is: \{davinci-fundamental\}"
\item \textbf{davinci-error-tail}: ``\{Text\} The common mistakes are: \{davinci-error\}"
\end{itemize}

Furthermore, for each dataset, we denote the best performance among cot-tail, error-tail, and fundamental-tail as \textbf{teacher-analysis}, while the best performance among davinci-cot-tail, davinci-error-tail, and davinci-fundamental-tail as \textbf{davinci-analysis}.

% TODO: 排版太丑了

\subsubsection{Student Model And Evaluation}
We chose the \textbf{bloomz-7.1b}\footnote{https://huggingface.co/bigscience/bloomz-7b1} model with intermediate accuracy as the student model. For evaluating each dataset's test split, we used the \textbf{lm-evaluation-harness}\footnote{https://github.com/EleutherAI/lm-evaluation-harness} method. Specifically, we write new tasks for all datasets and evaluate full checkpoints of finetuned student model through zero-shot multiple-choice questions, obtaining its total accuracy.

Apart from the above, other settings, including hyperparameters and training GPU, are in the appendix.
% TODO 引用格式
% TODO 确定 GPU 是不是这么写，引用 appendix
% Hyperparameter setting 貌似在 appendix

\subsection{Finetuning Results}
For each task type in five datasets, we finetuned the student model with 50 epochs and evaluated the accuracy of each checkpoint, ending in 2000 results. We show the Training fluctuations in \ref{fig:fluctuations} and best results in \ref{tab:best}.

% 这里似乎没有表达清楚我们 finetune 的方式
\input{table/best.tex}
\input{figure/fluctuations.tex}

% 图全部重画，都挂了

\subsubsection{Compared with manual CoT} Comparing finetune performance on manual-tail and cot-tail, the TeacherLM's cot-tail surpassed human annotation (manual-tail) on three out of five datasets (ECQA, QASC, and StrategyQA). In full consideration of teacher-analysis, it has clear advantages on four out of five datasets (CREAK, ECQA, QASC, and StrategyQA), which indicates that the TeacherLM's data enhancement ability on a single task rivals or exceeds artificial.

% 这一段的结尾 Grammarly 报错，但是我觉得没问题
% 这一段是否要给出确切的数据指标？

\subsubsection{Compared with text-davinci-003} 
We have already seen that the TeacherLM's performance on MMLU has surpassed most of the hundred billion parameters LLMs. However, ``It is better to teach someone how to fish than to give them the fish." Hence we want to further compete the TeacherLM's data enhancement ability with these hundred billion parameters LLMs. The latest GPT-3 model, text-davinci-003, is said to be the most potent generate LLM ever, so we chose it as our baseline model.

% TeacherLM 貌似是专有名词，需要加入 the

Comparing the performance of teacher-analysis and davinci-analysis, we find that teacher-analysis works better on StrategyQA and CREAK, and they perform the same on SenseMaking. Regarding the text-davinci-003's enormous model size, the TeacherLM has a comparable data enhancement ability and more parameter efficiency.

\subsubsection{Mitigate the Adversity of CoT Hurt}
In previous literature, researchers denote the situation when manual-tail performs worse than text as \textbf{CoT Hurt}, which indicates the task itself is so tricky that manually annotated chain-of-thought does not provide any help or even do harm to the performance. We find remarkable CoT Hurt on ECQA, QASC, and StrategyQA. Human analysis of these datasets hurt the student model's performance. However, cot-tail always performs better than manual-tail on these datasets, indicating that the teacherLM's data enhancement mitigates the CoT Hurt adversary and even completely reverses the CoT Hurt on QASC and StrategyQA, with cot-tail performing higher than text.

% 加入引用


\subsection{Human Evaluation}
%qinruoyu
The accuracy of student model is just part of the TeacherLM's data enhencement ability, hence we continue to evaluate the quality of fundamentals, chain of thought, and common mistakes at the finer-grained feature level. We performed a human evaluation experiment to assess the absolute quality of human annotations and the TeacherLM's analysis, with three different human judges to separately score the TeacherLM's analysis and human annotations for the same 600 samples over [TODO] datasets. For each sample, the judges were asked to give scores of 1-10 on the following aspects: (1) Fluency; (2) Consistency; (3) Factuality; (4) Sufficiency of Information; (5) Minimality; (6) Correlation; (7) Logical Coherence; (8) Overall Quality. The human rater instructions are given in section \ref{sec:appendix}.
% 

\begin{table}[t]
    % \vskip -0.05in
    \caption{Human evaluation results for explanations generated by TeacherLM and human. Numbers are averaged over 3 judges. SI: Sufficiency of Information and LC: Logical Coherence.}
    \label{tab:human-evaluation}
    \vskip 0.05in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcccr}
    \toprule
    Aspect   & Human & TeacherLM\\
    \midrule
    Fluency & 10 & 10 \\
    Consistency & 10 & 10\\
    Factuality & 10 & 10\\
    SI & 10 & 10\\
    Minimality & 10 & 10\\
    Correlation & 10 & 10\\
    LC & 10 & 10\\
    Overall & 10 & 10\\
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.05in
    \vskip -0.1in
\end{table}

The results of this human evaluation are shown in Table~\ref{tab:human-evaluation}~—[TODO: analysis].


==> content/introduction.tex <==
Large Language Models have recently revolutionized the NLP landscape \cite{brown2020language,rae2021scaling,chowdhery2022palm,wei2022emergent}. Compared to the increase in model size, an essential thing for achieving a deeper understanding of language is to utilize data effectively. The key to enhancing the capabilities of language models lies in effectively teaching them to comprehend and use the data provided, with related work primarily divided into task-level and instance-level. 
% 首先，这里应该是 a key 而不是 the key 吧，因为这不是唯一路径；其次，我感觉模型的任何训练过程都是在 comprehend and use the data provided，只有 Instruction Finetune 才会在意 task-level and instance-level，所以改成 teaching (finetuning) them to comprehend and use the data provided through prompts or instructions

Task-level data augmentation, primarily focused on instruction tuning, has pushed the generality of language models to new heights when combined with multi-task training \cite{wei2021finetuned,ouyang2022training,sanh2021multitask,wang2022benchmarking,chung2022scaling,taylor2022galactica,muennighoff2022crosslingual,iyer2022opt}, resulting in stronger zero-shot and few-shot capabilities. However, this is just the beginning as a new stage will flourish in instance-level data enhancement. Retrieval-based pre-trained language models \cite{borgeaud2021improving,izacard2022few} can rival the abilities of larger language models by utilizing smaller models in conjunction with massive databases. 
% 前文讲的是 Task-level teaching，这里主语突然换成 Task-level data augmentation 比较突兀，我认为 Task-level finetuning with corresponding data augmentation。
% 不要用将来时吧，就使用 a new stage flourish in instance-level data enhancement。
% Retrieval-based pre-trained language models 前面缺少转折，比如加上一个 For this purpose, 

The large language model (LLM) is an excellent teacher \cite{wang2021towards,ho2022large}, and it can generate relevant information for each sample, which enables the student model to produce significant benefits after training on enhanced data. The combination of the chain of thought and in-context learning has unlocked more vital reasoning abilities for LLMs \cite{wei2022chain,suzgun2022challenging,lampinen2022can}, guiding models to think critically rather than searching for information in their memory.
% 同样，这里 The large language model 前也缺乏转折，比如加上 On the other hand, The large language model is also an excellent teacher
% training 改成 finetuning 吧
% rather than merely searching for information in their memory 加入 merely
Adding the sentence ``Let's think step by step'' before LLMs generate an answer can induce the model to generate a step-by-step chain of thought and significantly improve the model's accuracy in solving reasoning tasks \cite{kojima2022large}. Therefore, it can be said that large language models are zero-shot reasoners, and they can also be considered zero-shot data enhancement generators.
% improve the model's accuracy in solving reasoning tasks 的 the 可以删了，语言简练些
% Therefore, LLMs are zero-shot reasoners and can also be considered zero-shot data enhancement generators.

``It is better to teach someone how to fish than to give them the fish." This adage applies to language models as well. The question then arises, how can we effectively teach a language model? The answer is to allow the language model to learn in a way that mimics how humans learn. Simply providing a label with a straightforward answer is insufficient for many NLP tasks.
Instead, we aim to shift the learning objectives of language models from results-oriented to process-oriented, moving away from rote memorization and towards a more holistic understanding to break through the limitations currently imposed on language model capabilities. 

In order to achieve this, we define the learning process as comprising three dimensions: fundamental, chain of thought, and common mistake. Our ultimate goal is for every sample in an NLP dataset to be annotated with this information.
% TODO 我改成这样：Our ultimate goal is to annotate this information for every sample in an NLP dataset.
However, current retrieval-based language models and existing large language models cannot provide comprehensive information and would incur high computational costs. To address this, we propose TeacherLM, which is specifically designed for this purpose.

To ensure that TeacherLM has strong zero-shot capabilities for most natural language processing tasks, we have collected 2 million samples from multiple domains for training. We have combined manual annotation and STaR strategy to construct a complete question-answer-fundamental-chain of thought-common mistake five-element for each sample.
% 删去 . We have 改成 and

In sum, our key contributions are:
% TODO 这个不是 in sum 吧，in sum 是总结前文，这里应该是 in shot？
\begin{itemize}
\item \textbf{Comprehensive}:
TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information that can be tailored to the characteristics of the task, allowing each task to learn the most suitable knowledge.
% TODO 我改了改 TeacherLM can explain fundamentals, chain of thought, and common mistakes, providing comprehensive information tailored to the characteristics of the task and allowing language models to learn the most relevant knowledge of each task.
\item \textbf{Generalizability}:
TeacherLM is suitable for a variety of datasets and models. We enhanced 59 NLP datasets and then used various parameter models of Opt and Bloom as student models for multi-task training on the enhanced data, as shown in the figure. Compared to non-enhanced versions, the zero-shot scores for MMLU, QASC, SenseMaking, CREAK, StrategyQA, and ECQA improved by more than 10\%.
\item \textbf{Fight big with small}:
TeacherLM-7.1B model achieved a zero-shot score of 52.3 on MMLU, surpassing the majority of the hundreds of billions of parameter models.
% TODO surpassing most of the hundred billion parameter models. 
\item \textbf{Beyond human annotation}:
On the QASC, SenseMaking, CREAK, StrategyQA, and ECQA datasets, TeacherLM-7.1B has demonstrated the ability to enhance data beyond human annotation and has some competitiveness compared to text-davinci-003, and to a great extent mitigates the CoT hurt situation.
% TODO 这一段我觉得写的有问题，五个数据集只能说大部分超过，部分媲美，而不是完全 beyond。
% 后面关于 some competitiveness 不如改成 clear competitiveness。
% CoT hurt 的 hurt 是大写吧，比如 CoT Hurt。
% text-davinci-003 需要加引用
\item \textbf{Low cost and low resource consumption}:
TeacherLM-7.1B has only 7.1 billion parameters; compared to models such as text-davinci-003, it has efficient inference speed and lower running configuration requirements. Therefore, with the significant cost reduction, we can augment NLP datasets of millions of levels, further opening the door to the reasoning world.
% 这里的标题提啊长了，改成 Convenient and cost effective

\item \textbf{Open source}:
We will release the TeacherLM series of models and augmented datasets as open-source.
\end{itemize}


==> content/train_teacher_store.tex <==

\input{figure/acc_mmlu.tex}
\input{table/TeacherLM_multistage.tex}
A good teacher can be a beacon, guiding students toward mastering the methods to solve problems. We want the same for the TeacherLM. In this regard, we make two primary efforts. Firstly, we construct a dataset comprising two million detailed explanations. Secondly, we adopt a multi-stage progressive training mode, moving from generality towards specialization.
% want -> aim
\subsection{Dataset Construction}

\textbf{P3-Sense-3K}
We extract 58 supervised datasets from P3 \cite{sanh2021multitask}. Each dataset contains multiple prompts, resulting in 529 tasks. To ensure sample balance, We select at most 3,000 samples of length less than 1,200 for each task. There are 1,400,364 samples in total. Then we format multiple choice tasks in the form of ``\textit{Q: \{question\} \{options\} A: \{answer\}}''. All other tasks are changed to the form of ``\textit{Q: \{question\} A: \{answer\}}''.

\textbf{Muffin-3W}
We extract 56 supervised datasets from Muffin \cite{wei2021finetuned}, and each dataset includes ten prompts. Similarly, We select at most 30,000 samples of length less than 1,200 for each task. There are 1,155,767 samples in total. All tasks are changed to the form of ``\textit{Q: \{question\} A: \{answer\}}''.

% 1200 tokens 么？

\textbf{TeacherData-2M}
Furthermore, we collect 2 million pieces of multi-domain data not included in any public datasets for training. We utilize manual annotation, and the STaR \cite{zelikman2022star} strategy to construct a five-element fixed paradigm for each sample, including the question, answer, fundamentals, chain of thought, and common mistakes. We select samples of length less than 2048.

% 这里要不要引用 intro 或者和 intro 统一？
% We utilize manual annotation and the STaR \cite{zelikman2022star} 

\subsection{Training Procedure}
Training the teacher models aims to obtain checkpoints that generalize well and can generate augmentations. In this section, we introduce our base models and the details of the multi-stage training.
% Training the teacher models aims to obtain checkpoints excelling at generating comprehensive explanations with solid generalization.
\subsubsection{Models}
In this work, our base models are the BLOOM \cite{scao2022bloom} series ranging from 560 million to 176 billion parameters, which are pre-trained on the ROOTS \cite{laurenccon2022bigscience} corpus in 46 natural languages and 13 programming languages. BLOOM models are large decoder-only language models pre-trained for 350 billion tokens.
%For each model, we adopt different hyperparameter settings. The rest of the training process is precisely the same. 

% parameters 需要介绍吧

\subsubsection{Multi-stage training}
For each model, we adopt a multi-stage training procedure. 

\textbf{Multi-task training}
Previous literature has shown that training on a large number of tasks with instructions can improve the model's zero-shot ability and allow it to generalize well on unseen tasks \cite{sanh2021multitask, wei2021finetuned}. Therefore, We use P3-Sense-3K and Muffin-3W to conduct multitask training. We combine the two mixtures.

\textbf{Personalization training}
Using the TeacherData-2M dataset, the model simultaneously learns to analyze each sample's fundamentals, chain of thought, and common mistakes. Through this process, the models can generate three types of content.

\textbf{Specialization learning}
We split the TeacherData-2M dataset and train three independent models to focus on learning fundamentals, chain of thought, and common mistakes, respectively. The resulting models are referred to as TeacherLM-Fundamental, TeacherLM-COT, and TeacherLM-CommonMistake.

In each stage of training, we use packing \cite{raffel2020exploring} to combine multiple texts, and terminators separate different texts. The interaction between texts is eliminated by setting the attention mask and resetting the position id. Models of different sizes use different learning rates and batchsizes. According to the number of parameters from small to large, they are 3e-4/256(TeacherLM-560M), 1e-4/512(TeacherLM-1.1B), 4e-5/512(TeacherLM-3B), 2e-5/768(TeacherLM-7.1B), 6e-5/1024(TeacherLM-176B). After the first stage, the way to select checkpoints to continue training is to evaluate the performance on the MMLU \cite{hendrycks2020measuring} benchmark. The performance on the MMLU benchmark and the manual evaluation results are the reference for selecting checkpoints for the second and third stages.

%\begin{table}[t]
%\caption{Training hyperparameter settings for each model size. t1, t2, t3 represent the amount of data trained in the three stages.}
%\label{sample-table}
%\vskip 0.15in
%\begin{center}
%\begin{tabular}{lccccr}
%\toprule
%parameters & lr & bs & t1 & t2 &t3 \\
%\midrule
%560M    & 3e-4 & 256 & 5B & 7.5B & 0.5B\\
%1.1B & 1e-4 & 512 & 5B & 7.5B & 0.5B \\
%3B    & 4e-5 & 512 & 5B &7.5B & 0.5B \\
%7.1B    & 2e-5 & 768 & 0.5B & 8B & 1.5B  \\    
%\bottomrule
%\end{tabular}
%\end{center}
%\vskip -0.5in
%\end{table}


\input{figure/comparison.tex}
\subsection{Evaluation Protocol}
\subsubsection{Benchmark}
For the teacher models, we focus on the performance on the held-out tasks that are not included in the training procedure. Specifically, we evaluate the teacher models on the MMLU(57 tasks) benchmark in the zero-shot setting. The benchmark consists of exam-like questions on academic subjects such as mathematics, history, law, and medicine.

\subsubsection{Evaluation Method}
% The evaluation adopts the method of rank classification. In more detail, assume answers are from a fixed set $\mathbb{A}$, and $answer_i\in\mathbb{A}$, where $i=1,...,n$, $n$ indexes $n$ candidate answers. Calculate the probability of each candidate answer using the Formula \ref{eval}. $\log P(a_k|q,a_1,...,a_{k-1})$ is the log probability of generating the k-th token $a_k$ in $answer_i$ conditioned on the previous tokens. $K$ is the total number of tokens in $answer_i$ and $q$ is the question. Choose the answer with the highest probability and calculate average accuracy on all tasks.

The evaluation adopts the method of rank classification. In more detail, assume answers are from a fixed set $\mathbb{A}$, and $\text{answer}_i\in\mathbb{A}$, where $i=1,...,n$, $n$ indexes $n$ candidate answers. Calculate the probability of each candidate answer using the Formula: 
\begin{equation}
    \displaystyle P(\text{answer}_i|q)=\frac{1}{K}\sum_{k=1}^{K}\log P(a_k|q,a_1,...,a_{k-1})
\label{eval}
\end{equation}
Here $\log P(a_k|q,a_1,...,a_{k-1})$ is the log probability of generating the k-th token $a_k$ in $\text{answer}_i$ conditioned on the previous tokens. $K$ is the total number of tokens in $\text{answer}_i$ and $q$ is the question. Choose the answer with the highest probability and calculate average accuracy on all tasks.

    



% $$
%     P(\text{answer}_i|q)=\frac{1}{K}\sum_{k=1}^{K}\log P(a_k|q,a_1,...,a_{k-1})
% \label{eval}
% $$

%\begin{table}[t]
%\caption{Average MMLU scores (\%) for 57 tasks with model and human accuracy comparisons.}

%\vskip 0.15in
%\begin{center}
%\begin{tabular}{lcr}
%\toprule
%model & parameters & MMLU \\
%\midrule
%TeacherLM    & 560M & 38.24 \\
%TeacherLM & 1.1B & 41.38 \\
%TeacherLM    & 3B & 46.74 \\
%TeacherLM    & 7.1B & 52.3  \\    
%PaLM(5-shot)     & 8B & 24.3 \\
%BLOOM(5-shot)        & 176B &31.9 \\
%Average Human &-&34.5 \\
%FLAN-PaLM(5-shot)      & 8B & 49.3 \\  
%PaLM(5-shot)      & 62B & 55.1  \\
%FLAN-PaLM(5-shot)   & 62B & 59.6 \\
%\bottomrule
%\end{tabular}
%\end{center}
%\vskip -0.1in
%\end{table}
\subsection{Results}
\subsubsection{Zero-shot Setting}
We show the MMLU scores with model and human comparisons in Figure \ref{mmlu-figure}. There are some key points.

First, models with few parameters can still benefit from our datasets. Even our 560M model exceeds BLOOM-176B. Moreover, scaling the CoT data to a larger size can improve zero-shot performance. In FLAN-PaLM \cite{chung2022scaling}, nine CoT datasets are added to improve the performance on the held-out tasks. When we scale the number of CoT samples to 2 million, we can see that the improvement is fantastic. The TeacherLM-7.1B model has achieved a zero-shot score of 52.3 on the MMLU, surpassing the 5-shot performance of the hundred billion parameter models. Additionally, the zero-shot score of TeacherLM-176B is 59.8, comparable to the 5-shot score of gopher-280B \cite{rae2021scaling}.

\subsubsection{Multi-stage Training Helps A Lot}
We show the evaluation results during multi-stage training in Table \ref{multi-stage-result}. In contrast to staged training, we also mixed all datasets and trained on them directly. The training hyperparameters and the number of steps are consistent. We find that directly blending all datasets scores much lower than multi-stage training. However, only the models using CoT data obtained continuous improvement in the third stage. This may indicate that tasks of the MMLU benchmark require higher reasoning ability. 
\subsubsection{Add Subject To Prompt}
Inspired by the fact that the MMLU benchmark is composed of different subject tasks, we added the prompt "\textit{The following are multiple choice questions (with answers) about \{subject\_name\}}" at the beginning of each text. We labeled the subject of each sample of TeacherData-2M. This approach increases the score of TeacherLM-7.1B by 2\%. We think such a prompt is more helpful for the model to use the correct knowledge to answer the question.



==> content/training_teacherlm_zmj.tex <==
A good teacher can be a beacon, guiding students toward mastering the correct learning methods. In this regard, we have made two primary efforts. Firstly, we have constructed a dataset comprising two million detailed explanations, which is used for training TeacherLM. Secondly, we adopted a multi-stage progressive training mode, moving from generality towards specialization.

\subsection{Datasets Construction}

\textbf{P3-sense-3k}
% 这个地方其实最好用 paragraph 而不是单纯的 textbf
 We have extracted 58 supervised datasets from P3. Each dataset contains multiple prompts, resulting in xxx tasks. To ensure sample balance, we have selected 3,000 samples per task with token lengths of less than 1,200, thus we formatted multiple choice tasks in the format of "question-options-answer" as shown in [figure], while keeping other tasks unchanged, containing [number] samples with a total token count of approximately [number].

\textbf{Muffin-3W}
We also extracted xxx supervised datasets from Muffin, each dataset includes ten prompts, and similarly, to ensure sample balance, we selected 30,000 samples per dataset with token length of less than 1200. The total dataset contains [number] samples, with a total token count of approximately [number].

\textbf{TeacherData-2M}
Furthermore, we collected 2 million pieces of multi-domain data that were not included in any public datasets for training. We then combined manual annotation and the STaR strategy to construct a five-element fixed paradigm for each sample, including question, answer, the fundamental, chain of thought, and common mistakes. We selected samples with token count less than 2048, resulting in a total token count of approximately xxx.
% the fundamentals 要用复数

\subsection{Models}
In this work, we use the BLOOM models ranging from 560 million to 176 billion parameters, which were pretrained on the ROOTS corpus in 46 natural languages and 13 programming languages. BLOOM models are large decoder-only language models pretrained for around 350 billion tokens with an architecture similar to GPT-3. 
% 数据集需要加入引用

\subsection{Multi-stage Training}
The training of TeacherLM is defined as four stages, gradually moving from generality to specialization.


\textbf{Pre-training}
% 这个地方其实最好用 paragraph 而不是单纯的 textbf
Utilizing a large corpus of general language data, which Bloom has already completed.

\textbf{Multitask training}
We use P3-sense-3k and Muffin-3W to conduct multitask training, cultivating the model's zero-shot abilities and allowing it to perform well on unseen tasks.

\textbf{Personalization training}
Using the TeacherData-2M dataset, the model simultaneously learns to analyze each sample's fundamentals, chain of thought, and common mistakes, thinking like a human.
% the model simultaneously learns to analyze each sample's fundamentals, chain of thought, and common mistakes, like a human. 去掉 thinking

\textbf{Specialization learning}
We split the TeacherData-2M dataset and trained three independent models to focus on learning fundamentals, chain of thought, and common mistakes, respectively. The resulting models are referred to as TeacherLM-Fundamental, TeacherLM-COT, and TeacherLM-CommonMistake.

\subsection{Evaluation methods and metrics}
The evaluation adopts the method of rank classification. Specifically, for each question, there is a set of alternative answers. Concatenate each candidate and question into text and input them into the model. We greedily choose the highest-likelihood answer from the set and score the model’s accuracy. 

In more detail, assume answers are from a fixed set $\mathbb{A}$, and $answer_i\in\mathbb{A}$, where $i=1,...,n$, $n$ indexes $n$ candidate answers. Calculate the probability of each candidate's answer using the formula (1). $logP(a_k|question,a_1,...,a_{k-1})$ is the log probability of generating the k-th token $a_k$ in $answer_i$ conditioned on the previous tokens, and $K$ is the total number of tokens in $answer_i$. Choose the answer with the highest probability.
\begin{equation}
    P(answer_i|question)=\frac{1}{K}\sum_{k=1}^{K}logP(a_k|question,a_1,...,a_{k-1})
\end{equation}
\input{figure/acc_mmlu.tex}

\subsection{Results}
The Massive Multitask Language Understanding (MMLU) benchmark consists of exam-like questions on academic subjects such as mathematics, history, law, and medicine.

As shown in Figure x, the TeacherLM-7.1B model has achieved a 0-shot score of 52.3 in MMLU, surpassing the 5-shot performance of the hundred billion parameter models, despite being much smaller. Additionally, the 0-shot score of TeacherLM-176B is 59.8, comparable to the 5-shot score of gopher-280B.

As evidenced by Figure X, multi-stage training has resulted in a continued increase in the model's zero-shot ability. The Personalization training stage, in particular, has resulted in a remarkable improvement, with the 0-shot score of TeacherLM-7.1B in MMLU increasing from xxx to xxx. Therefore, we are confident in positioning the TeacherLM as a beacon-like teacher.


==> figure/model_series.tex <==
\begin{table}[]
\begin{tabular}{l|lll}
\begin{tabular}[c]{@{}l@{}}Model Size  →\\ Model Series ↓\end{tabular} & small & base & large \\ \hline
BLOOM                                                                  & 1.1b  & 3b   & 7.1b  \\
BLOOMZ                                                                 & 1.1b  & 3b   & 7.1b  \\
OPT                                                                    & 1.3b  & 2.7b & 6.7b 
\end{tabular}
\end{table}

==> table/benchmark_score/mmlu.tex <==
\begin{table}[]
\begin{tabular}{l|lllllllll}
           & BLOOM-1B1 & BLOOM-3B & BLOOM-7B1 & BLOOMZ-1B1 & BLOOMZ-3B & BLOOMZ-7B1 & OPT-1B3  & OPT-2B7  & OPT-6B7  \\ \hline
Pretrained & 0.231358  & 0.251197 & 0.24681   & 0.236858   & 0.351606  & 0.396187   & 0.248096 & 0.222222 & 0.248614 \\
Origin     & 0.258236  & 0.263102 & 0.328452  & 0.247531   & 0.288558  & 0.322113   & 0.278105 & 0.282967 & 0.310434 \\
Sense      & 0.310299  & 0.361149 & 0.392068  & 0.322245   & 0.386185  & 0.413013   & 0.331217 & 0.369629 & 0.391026 \\
C          & 0.328667  & 0.380803 & 0.425548  & 0.328329   & 0.401285  & 0.440433   & 0.357785 & 0.384355 & 0.422467 \\
C\_M       & 0.325101  & 0.373854 & 0.423095  & 0.330993   & 0.402274  & 0.441483   & 0.349189 & 0.383614 & 0.412768 \\
C\_M\_F    & 0.330112  & 0.37967  & 0.430011  & 0.334543   & 0.402818  & 0.446843   & 0.343468 & 0.393545 & 0.427094 \\
Shuffle    & 0.330917  & 0.382266 & 0.410429  & 0.329396   & 0.400698  & 0.441309   & 0.353492 & 0.382323 & 0.415852 \\
M          & 0.319007  & 0.372569 & 0.41482   & 0.327553   & 0.389658  & 0.430516   & 0.347862 & 0.380526 & 0.399386 \\
F          & 0.316792  & 0.3698   & 0.419972  & 0.326653   & 0.397276  & 0.434832   & 0.331896 & 0.378718 & 0.409398 \\
F\_C\_M    & 0.325005  & 0.380491 & 0.431828  & 0.325694   & 0.402195  & 0.444557   & 0.333901 & 0.39519  & 0.422122
\end{tabular}
\label{tab:benchmark:mmlu}
\end{table}

==> table/best.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{cccccc}
    \toprule
& \textbf{CREAK}   & \textbf{ECQA}    & \textbf{QASC}    & \textbf{SenseMaking} & \textbf{StrategyQA} \\
\midrule
Text         & 76.73\% & \textbf{68.55\%} & 85.96\% & 79.10\%     & 72.37\%    \\
Manual       & 78.56\% & 49.64\% & 82.72\% & \textbf{82.09\%}     & 68.86\%    \\
Chain-of-Thought     & 75.86\% & 60.48\% & 89.96\% & 79.10\%     & 74.12\%    \\
Common Error & \textbf{78.99\%} & 64.95\% & \textbf{90.17\%} & 80.10\%     & 74.12\%    \\
Fundamental  & 75.78\% & 58.30\% & 84.13\% & 71.14\%     & \textbf{77.19\%}    \\
All          & 65.28\% & 51.96\% & 83.05\% & 78.11\%     & 68.86\%\\
\bottomrule
    \end{tabular}
    \caption{best results}
    \label{tab:best}
\end{table}
